Automatic DJ Transitions with Differentiable Audio Effects and Generative Adversarial Networks

A central task of a Disc Jockey (DJ) is to create a mixset of mu-sic with seamless transitions between adjacent tracks. In this paper, we explore a data-driven approach that uses a generative adversarial network to create the song transition by learning from real-world DJ mixes. In particular, the generator of the model uses two differentiable digital signal processing components, an equalizer (EQ) and a fader, to mix two tracks selected by a data generation pipeline. The generator has to set the parameters of the EQs and fader in such away that the resulting mix resembles real mixes created by humanDJ, as judged by the discriminator counterpart. Result of a listening test shows that the model can achieve competitive results compared with a number of baselines.

==> equations/mixer.tex <==
\begin{equation}
    \begin{split}
        & \hat{S_1}=S_1 \odot M_1(\theta_1)\\
        & \hat{S_2}=S_2 \odot M_2(\theta_2)
    \end{split}
    \label{eq:mixer}
\end{equation}

==> equations/relu1.tex <==
\begin{equation}
    ReLU1(\vec{v_{t}}) = min(max(0,\vec{v_{t}}), 1)
    \label{eq:relu1}
\end{equation}

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related work}
\paul{There are several research effort have made to tackle the problem of AI DJ in recent years which are mainly focus on two direction, reverse engineering and automatically creation.}

\paul{For reverse engineering, \cite{computational_dj} collected large-scale real-world DJ mixes and conducted mix-to-track subsequence alignment to extract important features such as cue points in the mix and corresponding start and endpoint in original paired tracks. Next, \cite{reverse_dj_transition} use the collected data to analyze DJ's musical action in the transition region [8]. Specifically, they extend the single-band analysis method proposed by \cite{reverse_dj} to the sub-band analysis method. Then, they assume all the DJ use the 3-bands equalizer with fixed low and high cut-off frequencies to composite their mix and apply a convex optimization approach to estimate the gain trajectories in each band. However, the approach may limit by the fixed cut-off frequencies and sub-band number of EQs. Furthermore, the approach is not used to generate new transitions but find the gain trajectories with best reconstructs mix given paired tracks}

\paul{For automatically creation, \cite{spotify_transition,highlight_dj,musicmixer} both tackle more than one issues in automatically DJ mix creation, but they all consider linear cross-fading as their transition strategy. \cite{drum&bass} is the first completed automatically DJ system which focus specific genre Drum & Bass. They manual set expert-rule which can deal with three types of transition. However, they indicate the rule is specific design for Drum & Bass instead of general purpose. \cite{user_adaptive_dj} include many different DJ technique to create transition, and used decision tree to decide which type of technique should be applied. However, they are pay more attention on adapt user preference instead of the quality. \cite{reinforcement_dj} propose a data-driven way to create transition by reinforcement learning. However, the model is guided to manipulate DJ mixer by multiple reward function based on DJ domain knowledge. For example, they penalize the transition with drastically change of volume and encourage all frequency bands to have similar amplitude which may not always the true in any situation \cite{drum&bass}. Moreover, they consider 3-bands EQs with fixed cut off frequencies as their DJ mixer which may be not the true for all the DJ mixer. Lastly, we do not consider it as our baseline because of lacking open source implementation.}
